A Conceptual Framework for Implicit Evaluation of Conversational Search Interfaces

Conversational search (CS) has recently become a significant focus of the information retrieval (IR) research community. Multiple studies have been conducted which explore the concept of conversational search. Understanding and advancing research in CS requires careful and detailed evaluation. Existing CS studies have been limited to evaluation based on simple user feedback on task completion. We propose a CS evaluation framework which includes multiple dimensions: search experience, knowledge gain, software usability, cognitive load and user experience, based on studies of conversational systems and IR. We introduce these evaluation criteria and propose their use in a framework for the evaluation of CS systems.

==> rough.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c}
 \hline 
    Measure & Description\\ \hline

    Average No. of Queries & - Total number of queries  \\
            & divided by total conversation \\  \hline
    %No. of Interactions & Subjects to fulfill their tasks \\ & with minimum expense and effort \\
    Average Query length & -Total query length\\ 
     & divided by number of \\ 
     & queries per conversations \\ \hline
    -No. of Document viewed & No. of document viewed\\ 
     & by the subject per conversation \\ \hline
    Markov Modeling & -Markov modeling can be \\ & used to determine the \\ & most probable sequences of \\ & actions by the subject \\ & -Can be compare with actual \\ 
    & sequence by the subject\\ \hline
    % & attitudes of the user to the product \\
    Average No. of turns & -Total number Turns \\ 
     & divided by total number \\ 
     & of conversation \\
  %  Other & -Variable discussed in table \ref{Interaction}\\ 
     %& attitudes of the user to the product \\
\hline
    \end{tabular}
      \caption{User engagements Variable in CS}
  \label{Interaction2}
\end{table}
